Safety Filtering While Training: Improving the Performance and Sample Efficiency of Reinforcement Learning Agents

Reinforcement learning (RL) controllers are flexible and performant but rarely guarantee safety. Safety filters impart hard safety guarantees to RL controllers while maintaining flexibility. However, safety filters can cause undesired behaviours due to the separation between the controller and the safety filter, often degrading performance and robustness. In this paper, we analyze several modifications to incorporating the safety filter in training RL controllers rather than solely applying it during evaluation. The modifications allow the RL controller to learn to account for the safety filter, improving performance. This paper presents a comprehensive analysis of training RL with safety filters, featuring simulated and real-world experiments with a Crazyflie 2.0 drone. We examine how various training modifications and hyperparameters impact performance, sample efficiency, safety, and chattering. Our findings serve as a guide for practitioners and researchers focused on safety filters and safe RL.

==> figs/real_experiments/ep_return.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=2.2in,
legend cell align={left},
legend style={
    fill opacity=0.6, 
    font=\footnotesize, 
    row sep=-1, 
    draw opacity=1, 
    text opacity=1, 
    draw=lightgray204, 
    at={(0.99,0.02)},
    anchor=south east,
},
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xlabel={Training Episodes},
xmin=-2, xmax=262,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Episode Return},
ymajorgrids,
ymin=64.7506739556706, ymax=354.99569918945,
ytick style={color=black}
]
\path [draw=limegreen, fill=limegreen, opacity=0.3]
(axis cs:10,164.750995277096)
--(axis cs:10,85.6985472753546)
--(axis cs:20,103.418676008483)
--(axis cs:30,146.785145600932)
--(axis cs:40,186.549255543627)
--(axis cs:50,196.813346108386)
--(axis cs:60,185.729110078038)
--(axis cs:70,208.925265905954)
--(axis cs:80,202.006162946998)
--(axis cs:90,207.947651575336)
--(axis cs:100,233.167586582763)
--(axis cs:110,220.489556626776)
--(axis cs:120,251.502244877711)
--(axis cs:130,272.171051205283)
--(axis cs:140,273.111769710861)
--(axis cs:150,271.301592205468)
--(axis cs:160,288.580916905067)
--(axis cs:170,288.459928298099)
--(axis cs:180,295.087676084263)
--(axis cs:190,295.640698050311)
--(axis cs:200,292.11669223675)
--(axis cs:210,293.645405181191)
--(axis cs:220,284.845597508593)
--(axis cs:230,285.520721404234)
--(axis cs:240,285.290025706787)
--(axis cs:250,283.051072825386)
--(axis cs:250,327.343738921254)
--(axis cs:250,327.343738921254)
--(axis cs:240,330.011198252201)
--(axis cs:230,330.927065495065)
--(axis cs:220,329.820015790937)
--(axis cs:210,331.236102898167)
--(axis cs:200,333.193887947363)
--(axis cs:190,329.674618550995)
--(axis cs:180,330.960125175216)
--(axis cs:170,319.689356803551)
--(axis cs:160,323.174582767717)
--(axis cs:150,327.711908324564)
--(axis cs:140,322.074464635523)
--(axis cs:130,317.976492505051)
--(axis cs:120,318.372862441284)
--(axis cs:110,311.320622992117)
--(axis cs:100,314.136698102672)
--(axis cs:90,315.747130953675)
--(axis cs:80,305.574402295081)
--(axis cs:70,317.268887678816)
--(axis cs:60,306.958517781441)
--(axis cs:50,248.224435153495)
--(axis cs:40,211.23861427206)
--(axis cs:30,186.647684119565)
--(axis cs:20,176.329711626899)
--(axis cs:10,164.750995277096)
--cycle;

\path [draw=darkgreen, fill=darkgreen, opacity=0.3]
(axis cs:10,157.561225436797)
--(axis cs:10,77.9436296481151)
--(axis cs:20,91.8643616588221)
--(axis cs:30,157.719989006605)
--(axis cs:40,178.629184003668)
--(axis cs:50,201.15769564081)
--(axis cs:60,231.478048339728)
--(axis cs:70,249.625725087539)
--(axis cs:80,278.362670242894)
--(axis cs:90,278.80730196866)
--(axis cs:100,291.821216285019)
--(axis cs:110,292.127324025332)
--(axis cs:120,293.595992910933)
--(axis cs:130,295.857360660503)
--(axis cs:140,289.829783613591)
--(axis cs:150,282.054886645888)
--(axis cs:160,294.032336478274)
--(axis cs:170,292.401688775861)
--(axis cs:180,306.779838766417)
--(axis cs:190,302.086750188909)
--(axis cs:200,306.946304944656)
--(axis cs:210,305.407867548579)
--(axis cs:220,305.647529834327)
--(axis cs:230,304.81245865016)
--(axis cs:240,299.671267444257)
--(axis cs:250,304.318026587535)
--(axis cs:250,316.991189972776)
--(axis cs:250,316.991189972776)
--(axis cs:240,318.191640698315)
--(axis cs:230,322.528535234412)
--(axis cs:220,318.938662399713)
--(axis cs:210,319.713678606695)
--(axis cs:200,326.626430807762)
--(axis cs:190,318.791435829625)
--(axis cs:180,319.917191394662)
--(axis cs:170,309.084974386256)
--(axis cs:160,323.193138471133)
--(axis cs:150,313.821791109722)
--(axis cs:140,315.769535200561)
--(axis cs:130,317.018937467814)
--(axis cs:120,309.336409351962)
--(axis cs:110,307.286891566881)
--(axis cs:100,308.728739397201)
--(axis cs:90,299.725034213349)
--(axis cs:80,304.083130158184)
--(axis cs:70,291.466130996145)
--(axis cs:60,297.506815951141)
--(axis cs:50,286.367221972698)
--(axis cs:40,259.289853751811)
--(axis cs:30,232.930748120997)
--(axis cs:20,220.827069663877)
--(axis cs:10,157.561225436797)
--cycle;

\path [draw=forestgreen, fill=forestgreen, opacity=0.3]
(axis cs:10,155.48476423511)
--(axis cs:10,89.2300842053385)
--(axis cs:20,142.175437272893)
--(axis cs:30,166.466409480655)
--(axis cs:40,182.718618876533)
--(axis cs:50,240.233647118426)
--(axis cs:60,250.536175589349)
--(axis cs:70,270.32809027445)
--(axis cs:80,299.216000421137)
--(axis cs:90,304.075285781151)
--(axis cs:100,306.757892109095)
--(axis cs:110,297.160310150244)
--(axis cs:120,287.2604430484)
--(axis cs:130,302.631370274403)
--(axis cs:140,300.629127763952)
--(axis cs:150,301.954802283145)
--(axis cs:160,309.604316550981)
--(axis cs:170,302.649372857197)
--(axis cs:180,317.693244808606)
--(axis cs:190,312.733743193634)
--(axis cs:200,321.601195331004)
--(axis cs:210,311.164935460022)
--(axis cs:220,313.63586670026)
--(axis cs:230,314.01224152745)
--(axis cs:240,308.741900898548)
--(axis cs:250,308.107994967161)
--(axis cs:250,327.118102043699)
--(axis cs:250,327.118102043699)
--(axis cs:240,327.112068751001)
--(axis cs:230,331.449583213803)
--(axis cs:220,329.873967431252)
--(axis cs:210,328.694092846145)
--(axis cs:200,331.018136086316)
--(axis cs:190,326.218444669671)
--(axis cs:180,324.791699243394)
--(axis cs:170,325.143756145822)
--(axis cs:160,330.753654558921)
--(axis cs:150,324.05883727564)
--(axis cs:140,320.12109690597)
--(axis cs:130,306.53183654115)
--(axis cs:120,307.638235058677)
--(axis cs:110,321.590589225832)
--(axis cs:100,318.433256118371)
--(axis cs:90,315.045243019932)
--(axis cs:80,315.31019696144)
--(axis cs:70,302.188686659628)
--(axis cs:60,303.68127010814)
--(axis cs:50,307.581702384869)
--(axis cs:40,296.107639615668)
--(axis cs:30,251.279970392791)
--(axis cs:20,217.111986440605)
--(axis cs:10,155.48476423511)
--cycle;

\path [draw=plum, fill=plum, opacity=0.3]
(axis cs:10,137.290274596059)
--(axis cs:10,78.821134617658)
--(axis cs:20,78.7185909028334)
--(axis cs:30,127.211608778175)
--(axis cs:40,176.946683495784)
--(axis cs:50,188.728017172379)
--(axis cs:60,196.698702895589)
--(axis cs:70,219.144679318745)
--(axis cs:80,234.276088634278)
--(axis cs:90,238.86504784983)
--(axis cs:100,293.260532890681)
--(axis cs:110,311.599541497693)
--(axis cs:120,317.93169798131)
--(axis cs:130,305.886121641513)
--(axis cs:140,321.068508558199)
--(axis cs:150,315.695694016522)
--(axis cs:160,312.67293560545)
--(axis cs:170,319.73529002703)
--(axis cs:180,325.36339901002)
--(axis cs:190,324.457890056217)
--(axis cs:200,321.376474647881)
--(axis cs:210,322.113427424155)
--(axis cs:220,324.391647055919)
--(axis cs:230,326.425945398965)
--(axis cs:240,319.757396963425)
--(axis cs:250,317.663953798708)
--(axis cs:250,340.321541999958)
--(axis cs:250,340.321541999958)
--(axis cs:240,335.222994853268)
--(axis cs:230,336.787800164599)
--(axis cs:220,341.802743497005)
--(axis cs:210,337.221426021368)
--(axis cs:200,331.756427368007)
--(axis cs:190,332.324386102294)
--(axis cs:180,331.805010951104)
--(axis cs:170,332.957669888108)
--(axis cs:160,331.758641419827)
--(axis cs:150,330.123154078545)
--(axis cs:140,330.698259447654)
--(axis cs:130,322.374021421349)
--(axis cs:120,325.882550885753)
--(axis cs:110,327.107212682408)
--(axis cs:100,325.306985369064)
--(axis cs:90,321.407920763538)
--(axis cs:80,320.042590111451)
--(axis cs:70,317.135618371952)
--(axis cs:60,324.504690819891)
--(axis cs:50,315.396487952138)
--(axis cs:40,303.450664930987)
--(axis cs:30,271.161651998873)
--(axis cs:20,183.748681661561)
--(axis cs:10,137.290274596059)
--cycle;

\path [draw=cornflowerblue, fill=cornflowerblue, opacity=0.3]
(axis cs:10,160.273213949857)
--(axis cs:10,79.9870281056647)
--(axis cs:20,141.020229865723)
--(axis cs:30,156.089681834352)
--(axis cs:40,195.151671997566)
--(axis cs:50,202.768734036213)
--(axis cs:60,235.644319863928)
--(axis cs:70,277.762337197255)
--(axis cs:80,266.036704476961)
--(axis cs:90,284.874317314949)
--(axis cs:100,282.121936167056)
--(axis cs:110,289.492746410832)
--(axis cs:120,290.23633477859)
--(axis cs:130,267.41046249578)
--(axis cs:140,297.20281220827)
--(axis cs:150,278.434894836451)
--(axis cs:160,280.329645242947)
--(axis cs:170,274.006833322531)
--(axis cs:180,265.935948798036)
--(axis cs:190,258.602445457319)
--(axis cs:200,292.087772899567)
--(axis cs:210,280.672272945466)
--(axis cs:220,285.508050692435)
--(axis cs:230,277.071432408032)
--(axis cs:240,275.187766132401)
--(axis cs:250,269.306528883505)
--(axis cs:250,299.521411968181)
--(axis cs:250,299.521411968181)
--(axis cs:240,318.155077412967)
--(axis cs:230,303.287933625888)
--(axis cs:220,322.062868005295)
--(axis cs:210,316.631904254006)
--(axis cs:200,320.701770533924)
--(axis cs:190,305.981126884277)
--(axis cs:180,310.20149163434)
--(axis cs:170,292.269780430817)
--(axis cs:160,307.31873332275)
--(axis cs:150,319.343159122032)
--(axis cs:140,314.284224115413)
--(axis cs:130,330.863093395432)
--(axis cs:120,320.28241527699)
--(axis cs:110,311.447816065147)
--(axis cs:100,314.312683435571)
--(axis cs:90,309.250476522306)
--(axis cs:80,317.033237916483)
--(axis cs:70,313.441453225311)
--(axis cs:60,324.770497227586)
--(axis cs:50,332.586939045641)
--(axis cs:40,304.263935447605)
--(axis cs:30,283.405003635778)
--(axis cs:20,244.499931699448)
--(axis cs:10,160.273213949857)
--cycle;

\addplot [semithick, limegreen]
table {%
10 123.827232347435
20 144.325167095126
30 170.762267358104
40 198.377842943666
50 220.967647918751
60 260.564257876502
70 272.223246926682
80 273.51174132142
90 284.00375945905
100 293.626331892553
110 288.618014543817
120 299.554873038296
130 303.199046893454
140 307.208244679624
150 305.947697459777
160 305.766186214083
170 307.247697436393
180 317.40528896451
190 318.298680421693
200 316.76080148811
210 316.021818748267
220 316.882255415199
230 319.159123344248
240 316.242987252326
250 315.197321078016
};
\addlegendentry{\textbf{Safe $\boldsymbol{\alpha=10^{-1}}$}}
\addplot [semithick, forestgreen]
table {%
10 122.360153759116
20 166.119561682996
30 207.476416739658
40 239.504432924195
50 273.196295629971
60 289.197652717355
70 287.664468972466
80 304.768920879286
90 310.227514305505
100 311.056211570145
110 304.561976889813
120 298.559551960649
130 304.952190961837
140 312.384686656081
150 312.060141136304
160 317.006824340333
170 314.478657131427
180 320.883185697829
190 319.931877991398
200 327.032717397971
210 322.532621430812
220 323.930901036097
230 324.253698023845
240 320.240612454782
250 316.1184683932
};
\addlegendentry{\textbf{Safe $\boldsymbol{\alpha=10^0}$}}
\addplot [semithick, darkgreen]
table {%
10 113.307815881225
20 162.725533521242
30 205.674241258704
40 235.801908787027
50 260.489226968085
60 276.833497765843
70 272.774834517447
80 292.245045839725
90 293.189371238731
100 299.365937945234
110 300.937806971535
120 301.828034781004
130 307.661920770312
140 304.036070681947
150 306.145921810571
160 307.791049976244
170 303.297952663465
180 312.755843694777
190 314.28990095913
200 315.943012572644
210 312.553485357147
220 312.040053393321
230 313.887391527975
240 312.238966102048
250 313.271696377394
};
\addlegendentry{\textbf{Safe $\boldsymbol{\alpha=10^1}$}}
\addplot [semithick, plum]
table {%
10 107.055229073639
20 134.310016860726
30 193.00663246545
40 230.928290534033
50 251.528470909732
60 279.100574635422
70 287.40992460465
80 295.219322516778
90 300.642464767801
100 310.560303698555
110 318.320817542108
120 321.406031237683
130 314.097863876012
140 326.187498273208
150 324.646114954076
160 323.565598831115
170 327.229968789423
180 328.241171957807
190 329.146678032853
200 327.709989754982
210 327.946974116289
220 331.41397802994
230 331.511872777062
240 328.014312734856
250 328.430266417243
};
\addlegendentry{Constr. Pen.}
\addplot [semithick, cornflowerblue]
table {%
10 118.479015695292
20 170.239992740727
30 225.426356544242
40 265.197050776913
50 284.673880356279
60 298.055441070958
70 303.479086440097
80 301.038153896624
90 300.023455209553
100 303.156804134978
110 299.807341000608
120 311.384735719625
130 310.159969061824
140 308.408527418296
150 302.807887415572
160 294.320932974739
170 284.593955872676
180 289.155071208694
190 291.684645988702
200 303.211341853282
210 294.709276743238
220 301.493959649837
230 292.115142050101
240 300.462609859513
250 285.425077674218
};
\addlegendentry{Standard}
\end{axis}

\end{tikzpicture}


==> figs/real_experiments/magnitude_of_correction.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=2.2in,
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xmin=0.5, xmax=5.5,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=45.0,anchor=east},
xticklabels={\textbf{Safe $\boldsymbol{\alpha=10^{-1}}$}, \textbf{Safe $\boldsymbol{\alpha=10^0}$}, \textbf{Safe $\boldsymbol{\alpha=10^1}$}, Standard, Constr. Pen.,,,,,,},
y grid style={darkgray176},
ylabel={Magnitude of Corrections},
ymajorgrids,
ymin=0, ymax=4.66820153120299,
ytick style={color=black}
]
\path [draw=black, fill=limegreen]
(axis cs:0.625,2.49177602887785)
--(axis cs:1.375,2.49177602887785)
--(axis cs:1.375,3.10347656065317)
--(axis cs:0.625,3.10347656065317)
--(axis cs:0.625,2.49177602887785)
--cycle;
\addplot [black]
table {%
1 2.49177602887785
1 2.31055050176649
};
\addplot [black]
table {%
1 3.10347656065317
1 3.44004641213647
};
\addplot [black]
table {%
0.8125 2.31055050176649
1.1875 2.31055050176649
};
\addplot [black]
table {%
0.8125 3.44004641213647
1.1875 3.44004641213647
};
\path [draw=black, fill=forestgreen]
(axis cs:1.625,1.91960986196431)
--(axis cs:2.375,1.91960986196431)
--(axis cs:2.375,2.13989514969853)
--(axis cs:1.625,2.13989514969853)
--(axis cs:1.625,1.91960986196431)
--cycle;
\addplot [black]
table {%
2 1.91960986196431
2 1.75679690875226
};
\addplot [black]
table {%
2 2.13989514969853
2 2.43598616334309
};
\addplot [black]
table {%
1.8125 1.75679690875226
2.1875 1.75679690875226
};
\addplot [black]
table {%
1.8125 2.43598616334309
2.1875 2.43598616334309
};
\path [draw=black, fill=darkgreen]
(axis cs:2.625,0.042029481182601)
--(axis cs:3.375,0.042029481182601)
--(axis cs:3.375,0.380113497882254)
--(axis cs:2.625,0.380113497882254)
--(axis cs:2.625,0.042029481182601)
--cycle;
\addplot [black]
table {%
3 0.042029481182601
3 0.0412372991744113
};
\addplot [black]
table {%
3 0.380113497882254
3 0.468684979590313
};
\addplot [black]
table {%
2.8125 0.0412372991744113
3.1875 0.0412372991744113
};
\addplot [black]
table {%
2.8125 0.468684979590313
3.1875 0.468684979590313
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
3 1.0524731017975
};
\path [draw=black, fill=cornflowerblue]
(axis cs:3.625,3.76926128482042)
--(axis cs:4.375,3.76926128482042)
--(axis cs:4.375,4.1124569987265)
--(axis cs:3.625,4.1124569987265)
--(axis cs:3.625,3.76926128482042)
--cycle;
\addplot [black]
table {%
4 3.76926128482042
4 3.54948946431445
};
\addplot [black]
table {%
4 4.1124569987265
4 4.44786990110639
};
\addplot [black]
table {%
3.8125 3.54948946431445
4.1875 3.54948946431445
};
\addplot [black]
table {%
3.8125 4.44786990110639
4.1875 4.44786990110639
};
\path [draw=black, fill=plum]
(axis cs:4.625,0.846865914172288)
--(axis cs:5.375,0.846865914172288)
--(axis cs:5.375,1.50598529001349)
--(axis cs:4.625,1.50598529001349)
--(axis cs:4.625,0.846865914172288)
--cycle;
\addplot [black]
table {%
5 0.846865914172288
5 0.766767337917709
};
\addplot [black]
table {%
5 1.50598529001349
5 2.22956237339275
};
\addplot [black]
table {%
4.8125 0.766767337917709
5.1875 0.766767337917709
};
\addplot [black]
table {%
4.8125 2.22956237339275
5.1875 2.22956237339275
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.625 2.89012804905711
1.375 2.89012804905711
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.625 2.04696221574771
2.375 2.04696221574771
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.625 0.0758574784455791
3.375 0.0758574784455791
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.625 3.96275162410699
4.375 3.96275162410699
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.625 0.866520768030105
5.375 0.866520768030105
};
\end{axis}

\end{tikzpicture}


==> figs/real_experiments/rate_of_change.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=2.2in,
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xmin=0.5, xmax=5.5,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=45.0,anchor=east},
xticklabels={\textbf{Safe $\boldsymbol{\alpha=10^{-1}}$}, \textbf{Safe $\boldsymbol{\alpha=10^0}$}, \textbf{Safe $\boldsymbol{\alpha=10^1}$}, Standard, Constr. Pen.,,,,,,},
y grid style={darkgray176},
ylabel={Rate of Change of Inputs},
ymajorgrids,
ymin=0, ymax=245.05845344203,
ytick style={color=black}
]
\path [draw=black, fill=limegreen]
(axis cs:0.625,230.445141266788)
--(axis cs:1.375,230.445141266788)
--(axis cs:1.375,236.894256727445)
--(axis cs:0.625,236.894256727445)
--(axis cs:0.625,230.445141266788)
--cycle;
\addplot [black]
table {%
1 230.445141266788
1 229.382598611224
};
\addplot [black]
table {%
1 236.894256727445
1 237.563306866123
};
\addplot [black]
table {%
0.8125 229.382598611224
1.1875 229.382598611224
};
\addplot [black]
table {%
0.8125 237.563306866123
1.1875 237.563306866123
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
1 200.639615619863
};
\path [draw=black, fill=forestgreen]
(axis cs:1.625,198.488617494278)
--(axis cs:2.375,198.488617494278)
--(axis cs:2.375,203.997539549074)
--(axis cs:1.625,203.997539549074)
--(axis cs:1.625,198.488617494278)
--cycle;
\addplot [black]
table {%
2 198.488617494278
2 197.419884286417
};
\addplot [black]
table {%
2 203.997539549074
2 205.288195085492
};
\addplot [black]
table {%
1.8125 197.419884286417
2.1875 197.419884286417
};
\addplot [black]
table {%
1.8125 205.288195085492
2.1875 205.288195085492
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
2 215.789481712509
};
\path [draw=black, fill=darkgreen]
(axis cs:2.625,146.525822766179)
--(axis cs:3.375,146.525822766179)
--(axis cs:3.375,156.171777754848)
--(axis cs:2.625,156.171777754848)
--(axis cs:2.625,146.525822766179)
--cycle;
\addplot [black]
table {%
3 146.525822766179
3 143.278625131839
};
\addplot [black]
table {%
3 156.171777754848
3 157.416557970066
};
\addplot [black]
table {%
2.8125 143.278625131839
3.1875 143.278625131839
};
\addplot [black]
table {%
2.8125 157.416557970066
3.1875 157.416557970066
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
3 170.893150848525
};
\path [draw=black, fill=cornflowerblue]
(axis cs:3.625,235.884543241868)
--(axis cs:4.375,235.884543241868)
--(axis cs:4.375,238.843939590856)
--(axis cs:3.625,238.843939590856)
--(axis cs:3.625,235.884543241868)
--cycle;
\addplot [black]
table {%
4 235.884543241868
4 235.509867384639
};
\addplot [black]
table {%
4 238.843939590856
4 239.838234870585
};
\addplot [black]
table {%
3.8125 235.509867384639
4.1875 235.509867384639
};
\addplot [black]
table {%
3.8125 239.838234870585
4.1875 239.838234870585
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
4 195.483255723113
};
\path [draw=black, fill=plum]
(axis cs:4.625,139.830683711228)
--(axis cs:5.375,139.830683711228)
--(axis cs:5.375,148.127650551909)
--(axis cs:4.625,148.127650551909)
--(axis cs:4.625,139.830683711228)
--cycle;
\addplot [black]
table {%
5 139.830683711228
5 135.433863441693
};
\addplot [black]
table {%
5 148.127650551909
5 148.720939975956
};
\addplot [black]
table {%
4.8125 135.433863441693
5.1875 135.433863441693
};
\addplot [black]
table {%
4.8125 148.720939975956
5.1875 148.720939975956
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.625 234.832236326045
1.375 234.832236326045
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.625 199.85973467449
2.375 199.85973467449
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.625 153.958183354915
3.375 153.958183354915
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.625 237.302274251965
4.375 237.302274251965
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.625 143.841579093706
5.375 143.841579093706
};
\end{axis}

\end{tikzpicture}


==> figs/real_experiments/reward.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{plum}{RGB}{221,160,221}

\begin{axis}[
height=2.2in,
tick align=outside,
tick pos=left,
width=3.5in,
x grid style={darkgray176},
xmin=0.5, xmax=5.5,
xtick style={color=black},
xtick={1,2,3,4,5},
xticklabel style={rotate=45.0,anchor=east},
xticklabels={\textbf{Safe $\boldsymbol{\alpha=10^{-1}}$}, \textbf{Safe $\boldsymbol{\alpha=10^0}$}, \textbf{Safe $\boldsymbol{\alpha=10^1}$}, Standard, Constr. Pen.,,,,,,},
y grid style={darkgray176},
ylabel={Experiment Return},
ymajorgrids,
ymin=0, ymax=329.385011935706,
ytick style={color=black}
]
\path [draw=black, fill=limegreen]
(axis cs:0.625,310.851589335647)
--(axis cs:1.375,310.851589335647)
--(axis cs:1.375,318.942209136969)
--(axis cs:0.625,318.942209136969)
--(axis cs:0.625,310.851589335647)
--cycle;
\addplot [black]
table {%
1 310.851589335647
1 309.923976799524
};
\addplot [black]
table {%
1 318.942209136969
1 325.859092264324
};
\addplot [black]
table {%
0.8125 309.923976799524
1.1875 309.923976799524
};
\addplot [black]
table {%
0.8125 325.859092264324
1.1875 325.859092264324
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
1 294.79899905037
};
\path [draw=black, fill=forestgreen]
(axis cs:1.625,314.978676220422)
--(axis cs:2.375,314.978676220422)
--(axis cs:2.375,317.499989495991)
--(axis cs:1.625,317.499989495991)
--(axis cs:1.625,314.978676220422)
--cycle;
\addplot [black]
table {%
2 314.978676220422
2 314.361274118559
};
\addplot [black]
table {%
2 317.499989495991
2 318.152174108578
};
\addplot [black]
table {%
1.8125 314.361274118559
2.1875 314.361274118559
};
\addplot [black]
table {%
1.8125 318.152174108578
2.1875 318.152174108578
};
\path [draw=black, fill=darkgreen]
(axis cs:2.625,305.426579475897)
--(axis cs:3.375,305.426579475897)
--(axis cs:3.375,306.419843326028)
--(axis cs:2.625,306.419843326028)
--(axis cs:2.625,305.426579475897)
--cycle;
\addplot [black]
table {%
3 305.426579475897
3 304.714309777023
};
\addplot [black]
table {%
3 306.419843326028
3 307.004293989796
};
\addplot [black]
table {%
2.8125 304.714309777023
3.1875 304.714309777023
};
\addplot [black]
table {%
2.8125 307.004293989796
3.1875 307.004293989796
};
\path [draw=black, fill=cornflowerblue]
(axis cs:3.625,258.854243151595)
--(axis cs:4.375,258.854243151595)
--(axis cs:4.375,272.260447739127)
--(axis cs:3.625,272.260447739127)
--(axis cs:3.625,258.854243151595)
--cycle;
\addplot [black]
table {%
4 258.854243151595
4 255.340698836699
};
\addplot [black]
table {%
4 272.260447739127
4 275.673714001338
};
\addplot [black]
table {%
3.8125 255.340698836699
4.1875 255.340698836699
};
\addplot [black]
table {%
3.8125 275.673714001338
4.1875 275.673714001338
};
\path [draw=black, fill=plum]
(axis cs:4.625,310.366878368308)
--(axis cs:5.375,310.366878368308)
--(axis cs:5.375,312.070070709751)
--(axis cs:4.625,312.070070709751)
--(axis cs:4.625,310.366878368308)
--cycle;
\addplot [black]
table {%
5 310.366878368308
5 309.099224176855
};
\addplot [black]
table {%
5 312.070070709751
5 312.913589934812
};
\addplot [black]
table {%
4.8125 309.099224176855
5.1875 309.099224176855
};
\addplot [black]
table {%
4.8125 312.913589934812
5.1875 312.913589934812
};
\addplot [black, mark=o, mark size=1.5, mark options={solid,fill opacity=0}, only marks]
table {%
5 299.490931959555
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.625 314.206699635712
1.375 314.206699635712
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.625 316.118912068041
2.375 316.118912068041
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.625 305.524554888185
3.375 305.524554888185
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.625 263.531571736939
4.375 263.531571736939
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.625 311.71564673199
5.375 311.71564673199
};
\end{axis}

\end{tikzpicture}


==> figs/simulation/parameter_ablation/rate_of_change.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{lightgreen}{RGB}{144,238,144}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{plum}{RGB}{221,160,221}
\definecolor{mediumorchid}{RGB}{186,85,211}
\definecolor{darkorchid}{RGB}{153,50,204}

\pgfdeclareplotmark{uncert}
{%
    \path[fill=lightgray204,postaction={pattern = north west lines, pattern color=black}] (-3\pgfplotmarksize,-2\pgfplotmarksize) rectangle (3\pgfplotmarksize,2\pgfplotmarksize);
}
\pgfdeclareplotmark{cert}
{%
    \path[fill=lightgray204] (-3\pgfplotmarksize,-2\pgfplotmarksize) rectangle (3\pgfplotmarksize,2\pgfplotmarksize);
}

\begin{axis}[
height=2.0in,
legend cell align={left},
legend style={
  fill opacity=0.6,
  draw opacity=1,
  text opacity=1,
  at={(0.01,0.98)},
  anchor=north west,
  draw=lightgray204,
  font=\footnotesize,
  row sep=-1,
},
tick align=outside,
tick pos=left,
width=3.4in,
x grid style={darkgray176},
xmin=0.3, xmax=8.7,
xtick style={color=black},
xtick={1,2,3,4,5,6,7,8},
xticklabel style={rotate=30.0,anchor=east, font=\footnotesize},
xticklabels={
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^{-1}}$},
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^0}$},
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^1}$},
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^2}$},
  Std. $\beta$$=$$0$,
  Std. $\beta$$=$$10^{-2}$,
  Std. $\beta$$=$$10^{-1}$,
  Std. $\beta$$=$$10^{0}$,
},
y grid style={darkgray176},
ylabel={Rate Of Change Of Inputs},
ymajorgrids,
ymin=0, ymax=65.5963166669011,
ytick style={color=black}
]
\addlegendimage{mark=cert,white}
\addlegendentry{Certified}
\addlegendimage{mark=uncert,white}
\addlegendentry{Uncertified}
\path [draw=black, fill=lightgreen]
(axis cs:0.6,7.63413992656598)
--(axis cs:1,7.63413992656598)
--(axis cs:1,11.5591181421502)
--(axis cs:0.6,11.5591181421502)
--(axis cs:0.6,7.63413992656598)
--cycle;
\addplot [black]
table {%
0.8 7.63413992656598
0.8 5.600498563602
};
\addplot [black]
table {%
0.8 11.5591181421502
0.8 17.0511610890257
};
\addplot [black]
table {%
0.7 5.600498563602
0.9 5.600498563602
};
\addplot [black]
table {%
0.7 17.0511610890257
0.9 17.0511610890257
};
\path [draw=black, fill=limegreen]
(axis cs:1.6,5.98252008256936)
--(axis cs:2,5.98252008256936)
--(axis cs:2,11.4077862860609)
--(axis cs:1.6,11.4077862860609)
--(axis cs:1.6,5.98252008256936)
--cycle;
\addplot [black]
table {%
1.8 5.98252008256936
1.8 3.97909157480848
};
\addplot [black]
table {%
1.8 11.4077862860609
1.8 18.8849637124403
};
\addplot [black]
table {%
1.7 3.97909157480848
1.9 3.97909157480848
};
\addplot [black]
table {%
1.7 18.8849637124403
1.9 18.8849637124403
};
\path [draw=black, fill=forestgreen]
(axis cs:2.6,2.72796627342635)
--(axis cs:3,2.72796627342635)
--(axis cs:3,5.65586539617897)
--(axis cs:2.6,5.65586539617897)
--(axis cs:2.6,2.72796627342635)
--cycle;
\addplot [black]
table {%
2.8 2.72796627342635
2.8 1.07212349153208
};
\addplot [black]
table {%
2.8 5.65586539617897
2.8 10.0108157010786
};
\addplot [black]
table {%
2.7 1.07212349153208
2.9 1.07212349153208
};
\addplot [black]
table {%
2.7 10.0108157010786
2.9 10.0108157010786
};
\path [draw=black, fill=darkgreen]
(axis cs:3.6,1.77111667253114)
--(axis cs:4,1.77111667253114)
--(axis cs:4,4.68037074808074)
--(axis cs:3.6,4.68037074808074)
--(axis cs:3.6,1.77111667253114)
--cycle;
\addplot [black]
table {%
3.8 1.77111667253114
3.8 0.633893514207326
};
\addplot [black]
table {%
3.8 4.68037074808074
3.8 8.99598779391583
};
\addplot [black]
table {%
3.7 0.633893514207326
3.9 0.633893514207326
};
\addplot [black]
table {%
3.7 8.99598779391583
3.9 8.99598779391583
};
\path [draw=black, fill=cornflowerblue]
(axis cs:4.6,8.15070742223021)
--(axis cs:5,8.15070742223021)
--(axis cs:5,40.1454026172359)
--(axis cs:4.6,40.1454026172359)
--(axis cs:4.6,8.15070742223021)
--cycle;
\addplot [black]
table {%
4.8 8.15070742223021
4.8 3.16956852144969
};
\addplot [black]
table {%
4.8 40.1454026172359
4.8 53.3672352440883
};
\addplot [black]
table {%
4.7 3.16956852144969
4.9 3.16956852144969
};
\addplot [black]
table {%
4.7 53.3672352440883
4.9 53.3672352440883
};
\path [draw=black, fill=plum]
(axis cs:5.6,6.75474492371633)
--(axis cs:6,6.75474492371633)
--(axis cs:6,14.4873720794181)
--(axis cs:5.6,14.4873720794181)
--(axis cs:5.6,6.75474492371633)
--cycle;
\addplot [black]
table {%
5.8 6.75474492371633
5.8 3.18371769482599
};
\addplot [black]
table {%
5.8 14.4873720794181
5.8 22.1074912326909
};
\addplot [black]
table {%
5.7 3.18371769482599
5.9 3.18371769482599
};
\addplot [black]
table {%
5.7 22.1074912326909
5.9 22.1074912326909
};
\path [draw=black, fill=mediumorchid]
(axis cs:6.6,3.59455357932809)
--(axis cs:7,3.59455357932809)
--(axis cs:7,6.98259094259575)
--(axis cs:6.6,6.98259094259575)
--(axis cs:6.6,3.59455357932809)
--cycle;
\addplot [black]
table {%
6.8 3.59455357932809
6.8 1.55161561390957
};
\addplot [black]
table {%
6.8 6.98259094259575
6.8 12.0576468046923
};
\addplot [black]
table {%
6.7 1.55161561390957
6.9 1.55161561390957
};
\addplot [black]
table {%
6.7 12.0576468046923
6.9 12.0576468046923
};
\path [draw=black, fill=darkorchid]
(axis cs:7.6,2.12736614927977)
--(axis cs:8,2.12736614927977)
--(axis cs:8,5.52555916156116)
--(axis cs:7.6,5.52555916156116)
--(axis cs:7.6,2.12736614927977)
--cycle;
\addplot [black]
table {%
7.8 2.12736614927977
7.8 0.880421890306409
};
\addplot [black]
table {%
7.8 5.52555916156116
7.8 10.6159020896775
};
\addplot [black]
table {%
7.7 0.880421890306409
7.9 0.880421890306409
};
\addplot [black]
table {%
7.7 10.6159020896775
7.9 10.6159020896775
};
\path [draw=black, fill=lightgreen, postaction={pattern=north west lines}]
(axis cs:1,2.36668229103088)
--(axis cs:1.4,2.36668229103088)
--(axis cs:1.4,7.29114305973053)
--(axis cs:1,7.29114305973053)
--(axis cs:1,2.36668229103088)
--cycle;
\addplot [black]
table {%
1.2 2.36668229103088
1.2 0.720477640628815
};
\addplot [black]
table {%
1.2 7.29114305973053
1.2 13.9284629821777
};
\addplot [black]
table {%
1.1 0.720477640628815
1.3 0.720477640628815
};
\addplot [black]
table {%
1.1 13.9284629821777
1.3 13.9284629821777
};
\path [draw=black, fill=limegreen, postaction={pattern=north west lines}]
(axis cs:2,1.96241870522499)
--(axis cs:2.4,1.96241870522499)
--(axis cs:2.4,5.24467647075653)
--(axis cs:2,5.24467647075653)
--(axis cs:2,1.96241870522499)
--cycle;
\addplot [black]
table {%
2.2 1.96241870522499
2.2 0.730762779712677
};
\addplot [black]
table {%
2.2 5.24467647075653
2.2 10.1160125732422
};
\addplot [black]
table {%
2.1 0.730762779712677
2.3 0.730762779712677
};
\addplot [black]
table {%
2.1 10.1160125732422
2.3 10.1160125732422
};
\path [draw=black, fill=forestgreen, postaction={pattern=north west lines}]
(axis cs:3,1.20767602324486)
--(axis cs:3.4,1.20767602324486)
--(axis cs:3.4,2.80188310146332)
--(axis cs:3,2.80188310146332)
--(axis cs:3,1.20767602324486)
--cycle;
\addplot [black]
table {%
3.2 1.20767602324486
3.2 0.594573140144348
};
\addplot [black]
table {%
3.2 2.80188310146332
3.2 5.12121391296387
};
\addplot [black]
table {%
3.1 0.594573140144348
3.3 0.594573140144348
};
\addplot [black]
table {%
3.1 5.12121391296387
3.3 5.12121391296387
};
\path [draw=black, fill=darkgreen, postaction={pattern=north west lines}]
(axis cs:4,1.06762900948524)
--(axis cs:4.4,1.06762900948524)
--(axis cs:4.4,2.02738577127457)
--(axis cs:4,2.02738577127457)
--(axis cs:4,1.06762900948524)
--cycle;
\addplot [black]
table {%
4.2 1.06762900948524
4.2 0.41693913936615
};
\addplot [black]
table {%
4.2 2.02738577127457
4.2 3.39092183113098
};
\addplot [black]
table {%
4.1 0.41693913936615
4.3 0.41693913936615
};
\addplot [black]
table {%
4.1 3.39092183113098
4.3 3.39092183113098
};
\path [draw=black, fill=cornflowerblue, postaction={pattern=north west lines}]
(axis cs:5,2.17889201641083)
--(axis cs:5.4,2.17889201641083)
--(axis cs:5.4,41.1884107589722)
--(axis cs:5,41.1884107589722)
--(axis cs:5,2.17889201641083)
--cycle;
\addplot [black]
table {%
5.2 2.17889201641083
5.2 0.985598862171173
};
\addplot [black]
table {%
5.2 41.1884107589722
5.2 62.4898567199707
};
\addplot [black]
table {%
5.1 0.985598862171173
5.3 0.985598862171173
};
\addplot [black]
table {%
5.1 62.4898567199707
5.3 62.4898567199707
};
\path [draw=black, fill=plum, postaction={pattern=north west lines}]
(axis cs:6,2.3403731584549)
--(axis cs:6.4,2.3403731584549)
--(axis cs:6.4,6.57146000862122)
--(axis cs:6,6.57146000862122)
--(axis cs:6,2.3403731584549)
--cycle;
\addplot [black]
table {%
6.2 2.3403731584549
6.2 1.13701009750366
};
\addplot [black]
table {%
6.2 6.57146000862122
6.2 12.8537349700928
};
\addplot [black]
table {%
6.1 1.13701009750366
6.3 1.13701009750366
};
\addplot [black]
table {%
6.1 12.8537349700928
6.3 12.8537349700928
};
\path [draw=black, fill=mediumorchid, postaction={pattern=north west lines}]
(axis cs:7,2.10499691963196)
--(axis cs:7.4,2.10499691963196)
--(axis cs:7.4,3.0716917514801)
--(axis cs:7,3.0716917514801)
--(axis cs:7,2.10499691963196)
--cycle;
\addplot [black]
table {%
7.2 2.10499691963196
7.2 0.84074079990387
};
\addplot [black]
table {%
7.2 3.0716917514801
7.2 4.49661111831665
};
\addplot [black]
table {%
7.1 0.84074079990387
7.3 0.84074079990387
};
\addplot [black]
table {%
7.1 4.49661111831665
7.3 4.49661111831665
};
\path [draw=black, fill=darkorchid, postaction={pattern=north west lines}]
(axis cs:8,1.3454518020153)
--(axis cs:8.4,1.3454518020153)
--(axis cs:8.4,2.15194594860077)
--(axis cs:8,2.15194594860077)
--(axis cs:8,1.3454518020153)
--cycle;
\addplot [black]
table {%
8.2 1.3454518020153
8.2 0.360657781362534
};
\addplot [black]
table {%
8.2 2.15194594860077
8.2 3.30141592025757
};
\addplot [black]
table {%
8.1 0.360657781362534
8.3 0.360657781362534
};
\addplot [black]
table {%
8.1 3.30141592025757
8.3 3.30141592025757
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.6 9.4216864296641
1 9.4216864296641
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.6 7.4671047363877
2 7.4671047363877
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.6 3.81002333953854
3 3.81002333953854
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.6 2.97302351563381
4 2.97302351563381
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.6 16.3706145415124
5 16.3706145415124
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
5.6 9.96191226432641
6 9.96191226432641
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
6.6 4.7219205641835
7 4.7219205641835
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
7.6 3.15458922142932
8 3.15458922142932
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1 4.57468056678772
1.4 4.57468056678772
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2 2.84928941726685
2.4 2.84928941726685
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3 1.91661024093628
3.4 1.91661024093628
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4 1.46514648199081
4.4 1.46514648199081
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
5 4.06125330924988
5.4 4.06125330924988
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
6 3.71904039382935
6.4 3.71904039382935
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
7 2.57456696033478
7.4 2.57456696033478
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
8 1.7257199883461
8.4 1.7257199883461
};
\end{axis}

\end{tikzpicture}


==> figs/simulation/parameter_ablation/reward.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{lightgreen}{RGB}{144,238,144}
\definecolor{forestgreen}{RGB}{34,139,34}
\definecolor{darkgreen}{RGB}{0,100,0}
\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{plum}{RGB}{221,160,221}
\definecolor{mediumorchid}{RGB}{186,85,211}
\definecolor{darkorchid}{RGB}{153,50,204}


\pgfdeclareplotmark{uncert}
{%
    \path[fill=lightgray204,postaction={pattern = north west lines, pattern color=black}] (-3\pgfplotmarksize,-2\pgfplotmarksize) rectangle (3\pgfplotmarksize,2\pgfplotmarksize);
}
\pgfdeclareplotmark{cert}
{%
    \path[fill=lightgray204] (-3\pgfplotmarksize,-2\pgfplotmarksize) rectangle (3\pgfplotmarksize,2\pgfplotmarksize);
}

\begin{axis}[
height=2.0in,
legend cell align={left},
legend style={
  fill opacity=0.6,
  draw opacity=1,
  text opacity=1,
  at={(0.99,0.02)},
  anchor=south east,
  draw=lightgray204,
  font=\footnotesize,
  row sep=-1,
},
tick align=outside,
tick pos=left,
width=3.4in,
x grid style={darkgray176},
xmin=0.3, xmax=8.7,
xtick style={color=black},
xtick={1,2,3,4,5,6,7,8},
xticklabel style={rotate=30.0,anchor=east, font=\footnotesize},
xticklabels={
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^{-1}}$},
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^0}$},
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^1}$},
  \textbf{\diffhl{Safe} $\boldsymbol{\alpha$$=$$10^2}$},
  Std. $\beta$$=$$0$,
  Std. $\beta$$=$$10^{-2}$,
  Std. $\beta$$=$$10^{-1}$,
  Std. $\beta$$=$$10^{0}$,
},
y grid style={darkgray176},
ylabel={Return},
ymajorgrids,
ymin=0, ymax=260,
ytick style={color=black}
]
\addlegendimage{mark=cert,white}
\addlegendentry{Certified}
\addlegendimage{mark=uncert,white}
\addlegendentry{Uncertified}
\path [draw=black, fill=lightgreen]
(axis cs:0.6,201.473382726431)
--(axis cs:1,201.473382726431)
--(axis cs:1,220.502023221104)
--(axis cs:0.6,220.502023221104)
--(axis cs:0.6,201.473382726431)
--cycle;
\addplot [black]
table {%
0.8 201.473382726431
0.8 173.440579260813
};
\addplot [black]
table {%
0.8 220.502023221104
0.8 235.715895801892
};
\addplot [black]
table {%
0.7 173.440579260813
0.9 173.440579260813
};
\addplot [black]
table {%
0.7 235.715895801892
0.9 235.715895801892
};
\path [draw=black, fill=limegreen]
(axis cs:1.6,203.475136778992)
--(axis cs:2,203.475136778992)
--(axis cs:2,222.214911298897)
--(axis cs:1.6,222.214911298897)
--(axis cs:1.6,203.475136778992)
--cycle;
\addplot [black]
table {%
1.8 203.475136778992
1.8 176.45147681403
};
\addplot [black]
table {%
1.8 222.214911298897
1.8 236.21929429843
};
\addplot [black]
table {%
1.7 176.45147681403
1.9 176.45147681403
};
\addplot [black]
table {%
1.7 236.21929429843
1.9 236.21929429843
};
\path [draw=black, fill=forestgreen]
(axis cs:2.6,198.929635700705)
--(axis cs:3,198.929635700705)
--(axis cs:3,219.080180716894)
--(axis cs:2.6,219.080180716894)
--(axis cs:2.6,198.929635700705)
--cycle;
\addplot [black]
table {%
2.8 198.929635700705
2.8 168.856834989595
};
\addplot [black]
table {%
2.8 219.080180716894
2.8 232.018904748963
};
\addplot [black]
table {%
2.7 168.856834989595
2.9 168.856834989595
};
\addplot [black]
table {%
2.7 232.018904748963
2.9 232.018904748963
};
\path [draw=black, fill=darkgreen]
(axis cs:3.6,191.842157714546)
--(axis cs:4,191.842157714546)
--(axis cs:4,210.16923637116)
--(axis cs:3.6,210.16923637116)
--(axis cs:3.6,191.842157714546)
--cycle;
\addplot [black]
table {%
3.8 191.842157714546
3.8 165.331005328397
};
\addplot [black]
table {%
3.8 210.16923637116
3.8 225.666525824954
};
\addplot [black]
table {%
3.7 165.331005328397
3.9 165.331005328397
};
\addplot [black]
table {%
3.7 225.666525824954
3.9 225.666525824954
};
\path [draw=black, fill=cornflowerblue]
(axis cs:4.6,188.184989742728)
--(axis cs:5,188.184989742728)
--(axis cs:5,215.132744775031)
--(axis cs:4.6,215.132744775031)
--(axis cs:4.6,188.184989742728)
--cycle;
\addplot [black]
table {%
4.8 188.184989742728
4.8 154.475970844549
};
\addplot [black]
table {%
4.8 215.132744775031
4.8 232.673823729289
};
\addplot [black]
table {%
4.7 154.475970844549
4.9 154.475970844549
};
\addplot [black]
table {%
4.7 232.673823729289
4.9 232.673823729289
};
\path [draw=black, fill=plum]
(axis cs:5.6,193.230159861583)
--(axis cs:6,193.230159861583)
--(axis cs:6,215.545660221483)
--(axis cs:5.6,215.545660221483)
--(axis cs:5.6,193.230159861583)
--cycle;
\addplot [black]
table {%
5.8 193.230159861583
5.8 161.863121492172
};
\addplot [black]
table {%
5.8 215.545660221483
5.8 232.934854411713
};
\addplot [black]
table {%
5.7 161.863121492172
5.9 161.863121492172
};
\addplot [black]
table {%
5.7 232.934854411713
5.9 232.934854411713
};
\path [draw=black, fill=mediumorchid]
(axis cs:6.6,199.884489473621)
--(axis cs:7,199.884489473621)
--(axis cs:7,218.846687964152)
--(axis cs:6.6,218.846687964152)
--(axis cs:6.6,199.884489473621)
--cycle;
\addplot [black]
table {%
6.8 199.884489473621
6.8 172.374620516941
};
\addplot [black]
table {%
6.8 218.846687964152
6.8 232.320064835196
};
\addplot [black]
table {%
6.7 172.374620516941
6.9 172.374620516941
};
\addplot [black]
table {%
6.7 232.320064835196
6.9 232.320064835196
};
\path [draw=black, fill=darkorchid]
(axis cs:7.6,186.125922864748)
--(axis cs:8,186.125922864748)
--(axis cs:8,209.509965477837)
--(axis cs:7.6,209.509965477837)
--(axis cs:7.6,186.125922864748)
--cycle;
\addplot [black]
table {%
7.8 186.125922864748
7.8 153.776400973238
};
\addplot [black]
table {%
7.8 209.509965477837
7.8 226.974427539481
};
\addplot [black]
table {%
7.7 153.776400973238
7.9 153.776400973238
};
\addplot [black]
table {%
7.7 226.974427539481
7.9 226.974427539481
};
\path [draw=black, fill=lightgreen, postaction={pattern=north west lines}]
(axis cs:1,7.32656023728543)
--(axis cs:1.4,7.32656023728543)
--(axis cs:1.4,23.5330894157801)
--(axis cs:1,23.5330894157801)
--(axis cs:1,7.32656023728543)
--cycle;
\addplot [black]
table {%
1.2 7.32656023728543
1.2 1.23757031960919
};
\addplot [black]
table {%
1.2 23.5330894157801
1.2 45.2297654829569
};
\addplot [black]
table {%
1.1 1.23757031960919
1.3 1.23757031960919
};
\addplot [black]
table {%
1.1 45.2297654829569
1.3 45.2297654829569
};
\path [draw=black, fill=limegreen, postaction={pattern=north west lines}]
(axis cs:2,14.1581365292061)
--(axis cs:2.4,14.1581365292061)
--(axis cs:2.4,70.624659504055)
--(axis cs:2,70.624659504055)
--(axis cs:2,14.1581365292061)
--cycle;
\addplot [black]
table {%
2.2 14.1581365292061
2.2 1.36498406927648
};
\addplot [black]
table {%
2.2 70.624659504055
2.2 154.284549674637
};
\addplot [black]
table {%
2.1 1.36498406927648
2.3 1.36498406927648
};
\addplot [black]
table {%
2.1 154.284549674637
2.3 154.284549674637
};
\path [draw=black, fill=forestgreen, postaction={pattern=north west lines}]
(axis cs:3,190.11549268523)
--(axis cs:3.4,190.11549268523)
--(axis cs:3.4,220.683204371086)
--(axis cs:3,220.683204371086)
--(axis cs:3,190.11549268523)
--cycle;
\addplot [black]
table {%
3.2 190.11549268523
3.2 145.865529015415
};
\addplot [black]
table {%
3.2 220.683204371086
3.2 240.099531559103
};
\addplot [black]
table {%
3.1 145.865529015415
3.3 145.865529015415
};
\addplot [black]
table {%
3.1 240.099531559103
3.3 240.099531559103
};
\path [draw=black, fill=darkgreen, postaction={pattern=north west lines}]
(axis cs:4,191.539362066681)
--(axis cs:4.4,191.539362066681)
--(axis cs:4.4,210.472579295644)
--(axis cs:4,210.472579295644)
--(axis cs:4,191.539362066681)
--cycle;
\addplot [black]
table {%
4.2 191.539362066681
4.2 166.884427101285
};
\addplot [black]
table {%
4.2 210.472579295644
4.2 229.598050639553
};
\addplot [black]
table {%
4.1 166.884427101285
4.3 166.884427101285
};
\addplot [black]
table {%
4.1 229.598050639553
4.3 229.598050639553
};
\path [draw=black, fill=cornflowerblue, postaction={pattern=north west lines}]
(axis cs:5,212.29110526931)
--(axis cs:5.4,212.29110526931)
--(axis cs:5.4,231.583308456183)
--(axis cs:5,231.583308456183)
--(axis cs:5,212.29110526931)
--cycle;
\addplot [black]
table {%
5.2 212.29110526931
5.2 184.673866296395
};
\addplot [black]
table {%
5.2 231.583308456183
5.2 246.260654270091
};
\addplot [black]
table {%
5.1 184.673866296395
5.3 184.673866296395
};
\addplot [black]
table {%
5.1 246.260654270091
5.3 246.260654270091
};
\path [draw=black, fill=plum, postaction={pattern=north west lines}]
(axis cs:6,220.298149243967)
--(axis cs:6.4,220.298149243967)
--(axis cs:6.4,234.26284719148)
--(axis cs:6,234.26284719148)
--(axis cs:6,220.298149243967)
--cycle;
\addplot [black]
table {%
6.2 220.298149243967
6.2 201.208660231159
};
\addplot [black]
table {%
6.2 234.26284719148
6.2 246.6074016949
};
\addplot [black]
table {%
6.1 201.208660231159
6.3 201.208660231159
};
\addplot [black]
table {%
6.1 246.6074016949
6.3 246.6074016949
};
\path [draw=black, fill=mediumorchid, postaction={pattern=north west lines}]
(axis cs:7,213.330051013599)
--(axis cs:7.4,213.330051013599)
--(axis cs:7.4,229.611048841962)
--(axis cs:7,229.611048841962)
--(axis cs:7,213.330051013599)
--cycle;
\addplot [black]
table {%
7.2 213.330051013599
7.2 189.847967555788
};
\addplot [black]
table {%
7.2 229.611048841962
7.2 244.121113408458
};
\addplot [black]
table {%
7.1 189.847967555788
7.3 189.847967555788
};
\addplot [black]
table {%
7.1 244.121113408458
7.3 244.121113408458
};
\path [draw=black, fill=darkorchid, postaction={pattern=north west lines}]
(axis cs:8,195.282365012286)
--(axis cs:8.4,195.282365012286)
--(axis cs:8.4,216.450079548215)
--(axis cs:8,216.450079548215)
--(axis cs:8,195.282365012286)
--cycle;
\addplot [black]
table {%
8.2 195.282365012286
8.2 165.68370522939
};
\addplot [black]
table {%
8.2 216.450079548215
8.2 232.637562009101
};
\addplot [black]
table {%
8.1 165.68370522939
8.3 165.68370522939
};
\addplot [black]
table {%
8.1 232.637562009101
8.3 232.637562009101
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
0.6 212.080527713124
1 212.080527713124
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1.6 214.107958400418
2 214.107958400418
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2.6 210.703053823205
3 210.703053823205
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3.6 202.359700734155
4 202.359700734155
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4.6 200.150191781747
5 200.150191781747
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
5.6 206.297693510961
6 206.297693510961
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
6.6 210.266466237547
7 210.266466237547
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
7.6 199.125662951788
8 199.125662951788
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
1 13.9219073862211
1.4 13.9219073862211
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
2 31.1881787863442
2.4 31.1881787863442
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
3 210.712815379098
3.4 210.712815379098
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
4 202.338849744561
4.4 202.338849744561
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
5 222.053714904166
5.4 222.053714904166
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
6 228.700983701576
6.4 228.700983701576
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
7 222.21494326843
7.4 222.21494326843
};
\addplot [line width=1pt, black, dash pattern=on 9.25pt off 4pt]
table {%
8 206.828006369195
8.4 206.828006369195
};
\end{axis}

\end{tikzpicture}

